Instruct2Attack: Language-Guided Semantic Adversarial Attacks

We propose Instruct2Attack (I2A), a language-guided semantic attack that generates semantically meaningful perturbations according to free-form language instructions. We make use of state-of-the-art latent diffusion models, where we adversarially guide the reverse diffusion process to search for an adversarial latent code conditioned on the input image and text instruction. Compared to existing noise-based and semantic attacks, I2A generates more natural and diverse adversarial examples while providing better controllability and interpretability. We further automate the attack process with GPT-4 to generate diverse image-specific text instructions. We show that I2A can successfully break state-of-the-art deep neural networks even under strong adversarial defenses, and demonstrate great transferability among a variety of network architectures.

==> figs/guidance.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figs/imgs/guidance.pdf}
    \caption{Illustration of adversarial guidance.}
    \label{fig:guidance}
\end{figure}

==> sec/X_suppl_alone.tex <==
\clearpage
\setcounter{page}{1}
\maketitlesupplementary
% \section{Background: Latent Diffusion Model}
% Diffusion models~\cite{sohl2015deep, ho2020denoising, nichol2021improved} are a family of generative models that model the target distribution by learning a reverse denoising generative process. A diffusion model consists of two processes: (1) a forward diffusion process that converts the input image $\xzero$ to noise map $\xT$ by gradually adding noise in $T$ forward steps; (2) a reverse denoising generative process that aims to recover $\vect{x}$ from $\xT$ by gradually denoising in $T$ reverse steps. 

% Instead of directly modeling the data distribution in the image space $\mathcal{X}$, latent diffusion models (LDMs)~\cite{rombach2022high} approximate the data distribution in a learned latent space $\mathcal{Z}=\{\vect{z}\ |\ \vect{z}=\mathcal{E}(\vect{x}), \vect{x}\in\mathcal{X}\}$, where $\mathcal{E}$ is an image encoder, and the images are reconstructed through an image decoder $\mathcal{D}: \Tilde{\vect{x}}=\mathcal{D}(\vect{z})$.  Given $\vect{z}_T\sim \mathcal{N}(\vect{0}, \sigma_{T}^{2}\vect{I})$, the reverse diffusion process of LDMs can be computed~\cite{song2021scorebased} as:
% \begin{equation}
%     \vect{z}_{t-1} = \vect{z}_{t} + (\sigma_{t}^{2} - \sigma_{t-1}^{2})\epsilon_{\theta}(\vect{z}_{t}, t) + \sqrt{\frac{\sigma_{t-1}^{2}(\sigma_{t}^{2} - \sigma_{t-1}^{2})}{\sigma_{t}^{2}}}\boldsymbol{\zeta}_{t},
% \end{equation}
% where $1\leq t \leq T$ is the time step, $\epsilon_{\theta}$ is the denoising network, $\sigma_t$ is the noise scale, and $\boldsymbol{\zeta}_t\sim \mathcal{N}(\vect{0}, \vect{I})$. 

% LDMs are capable of modeling conditional distributions~\cite{brooks2023instructpix2pix, rombach2022high} such as $p(\vect{z}|\vect{x}, \vect{T})$, where $\vect{x}$ is the input image, and $\vect{T}$ is the input text. This can be implemented with a conditional denoising network $\epsilon_{\theta}(\vect{z}_{t}, t, \vect{c}_{I}, \vect{c}_{T})$. Specifically, $\vect{x}$ is first encoded by the image encoder to obtain the image condition embedding $\vect{c}_{I}=\mathcal{E}(\vect{x})\in \mathbb{R}^{h \times w \times c}$ and $\vect{T}$ is encoded by a text encoder $\mathcal{C}$ to obtain the text condition embedding $\vect{c}_T=\mathcal{C}(\vect{I})\in \mathbb{R}^{m\times l}$. At each denoising step, $\vect{c}_{I}$ is concatenated with $\vect{z}_t$ as the input to $\epsilon_{\theta}$, while $\vect{c}_{T}$ is projected to the intermediate layers of $\epsilon_{\theta}$ via a cross-attention layer.
\renewcommand{\thefigure}{\Alph{figure}}
\renewcommand{\thetable}{\Alph{table}}
\setcounter{equation}{7}
\setcounter{table}{0}
\setcounter{figure}{0}
\section{Additional Implementation Details}
\subsection{Experiment Settings}
All experiments are conducted using the \texttt{PyTorch} framework. We fix the random seed of every experiment to avoid the randomness of diffusion sampling. 
\subsection{Projection Algorithm}
At the end of the attack generation, we ensure the perceptual constraint is satisfied by projecting $\vect{x}_{\text{adv}}$ back to the feasible set through dynamically adjusting $s_I$ and $s_T$ in Eq. (\textcolor{red}{3}) which control the trade-off between how strongly the edited image corresponds with the input image and the edit instruction. A higher $s_I$ produces an image that is more faithful to the input image, while a higher $s_T$ results in a stronger edit applied to the input. In this work, we use the default setting $s_I=1.5$ and $s_T=7.5$ suggested by~\cite{brooks2023instructpix2pix}. To project the adversarial image $\vect{x}_\text{adv}$ back to the LPIPS bound of $\gamma$, we first set $s_T=0$ and gradually increase the value of $s_I$ to find a value of $s_I^*$ such that the resulting image satisfies the LPIPS bound. Then we aim to increase the value of $s_T$ from 0 to find a $s_T^*$ that is as large as possible using the bisection method such that the final projected image satisfies the perceptual constraint. To search for $s_I^*$, we set the maximum value ${s_I}_\text{max}$ to 10, and the search step size $\eta_{s_I}$ to 0.2. To calculate $s_T^*$, we use $n=10$ iterations of the bisection method with the maximum value of $s_T$ set to ${s_T}_\text{max}=20$. The projection algorithm is summarized in~\Cref{alg:proj}. 

\begin{algorithm}[h]
\caption{Perceptual Projection}\label{alg:proj}
\begin{algorithmic}[1]
\State {\bfseries Input:} $\vect{x}$, $\vect{T}$, $\vect{z}_T$, $\gamma$, $T$, $\epsilon_\theta$, $\gE$, $\gD$, $\gC$,  optimized $\balpha$ and $\bbeta$, initial $s_I$, ${s_I}_\text{max}$, ${s_T}_\text{max}$, $\eta_{s_I}$, $n$.
\State {\bfseries Output:} Projected adversarial image $\Tilde{\vect{x}}_{\text{adv}}$ 
\LineComment{Image and text encoding}
\State $\vect{c}_I=\gE(\vect{x}),\ \ \vect{c}_L=\gC(\vect{L})$
\LineComment{Search for $s_I^*$} 
\State $s_T \gets 0$
\State {\bfseries while} $s_I \leq {s_I}_\text{max}$
\State $\ \ \ \ \Tilde{\vect{z}} =\text{LDM}(\vect{z}_T; \vect{c}_{I}, \vect{c}_{L}, \balpha, \bbeta, s_I, s_T$) \Comment{Sample $\Tilde{\vect{z}}$}
\State $\ \ \ \ \Tilde{\vect{x}}=\gD(\Tilde{\vect{z}})$ \Comment{Generate $\Tilde{\vect{x}}$}

\State \ \ \ \ {\bfseries if} $d(\Tilde{\vect{x}}, \vect{x})\leq \gamma$
\State \ \ \ \ \ \ \ \ $s_I^*=s_I$
\State \ \ \ \ \ \ \ \ {\bfseries break}
\State \ \ \ \ {\bfseries else}
\State \ \ \ \ \ \ \ \ $s_I = s_I + \eta_{s_I}$
\State \ \ \ \ {\bfseries end if} 
\State {\bfseries end while}

\LineComment{Calculate $s_T^*$} 
\State ${s_T}_\text{min} \gets 0$
\State {\bfseries for} $i=0$ \textbf{to} $n$
\State \ \ \ \  $s_T = ({s_T}_\text{min} + {s_T}_\text{max})/2$
\State $\ \ \ \ \Tilde{\vect{z}} =\text{LDM}(\vect{z}_T; \vect{c}_{I}, \vect{c}_{L}, \balpha, \bbeta, s_I^*, s_T$) \Comment{Sample $\Tilde{\vect{z}}$}
\State $\ \ \ \ \Tilde{\vect{x}}=\gD(\Tilde{\vect{z}})$ \Comment{Generate $\Tilde{\vect{x}}$}

\State \ \ \ \ {\bfseries if} $d(\Tilde{\vect{x}}, \vect{x}) > \gamma$
\State \ \ \ \ \ \ \ \ ${s_T}_\text{max}=s_T$
\State \ \ \ \ {\bfseries else}
\State \ \ \ \ \ \ \ \ ${s_T}_\text{min}=s_T$, $\Tilde{\vect{x}}_\text{adv} = \Tilde{\vect{x}}$
\State \ \ \ \ {\bfseries end if} 
\State {\bfseries end for}

\end{algorithmic}
\end{algorithm}



\subsection{Baseline Attacks}
The implementation details for the baseline attacks are as follows:
\begin{itemize}
    \item \textbf{FGSM}~\cite{szegedy2013intriguing}  We use $L_{\infty}$ norm with a bound of $4/255$.
    \item \textbf{PGD}~\cite{madry2018towards}:  We use $L_{\infty}$ norm with a bound of $4/255$ with 100 iterations and step size $1/255$.
    \item \textbf{MIM}~\cite{dong2018boosting}: We use $L_{\infty}$ norm with a bound of $4/255$ with 100 iterations, step size $1/255$, and decay factor $1.0$.
    \item \textbf{AutoAttack}~\cite{croce2020reliable}: We use $L_{\infty}$ norm with a bound of $4/255$ and use the \texttt{standard} version of AutoAttack\footnote{https://github.com/fra31/auto-attack}.
    \item \textbf{Fog}~\cite{kang2019testing}: We set the number of iterations to 200, $\epsilon$ to $128$, and step size to 0.002236.
    \item \textbf{Snow}~\cite{kang2019testing}: We set the number of iterations to 200, $\epsilon$ to $0.0625$, and step size to 0.002236.
    \item \textbf{Gabor}~\cite{kang2019testing}: We set the number of iterations to 200, $\epsilon$ to $12.5$, and step size to 0.002236.
    \item \textbf{StAdv}~\cite{xiao2018spatially}: We set the number of iterations to 200 with a bound of $0.005$.
    \item \textbf{PerC-AL}~\cite{zhao2020towards}: We follow the default settings in the official github repository\footnote{https://github.com/ZhengyuZhao/PerC-Adversarial}, and set the maximum number of iterations to 1000, $\alpha_l=1.0$, $\alpha_c=0.5$, and $\kappa=40$.
\end{itemize}
When applying EOT+BPDA attacks for adaptively attacking DiffPure in Sec. \textcolor{red}{4.2}, we set the maximum number of iterations to 50 for all attacks including I2A due to the high computational cost. 
\subsection{Victim Models for ImageNet}
The implementation details for the victim models of ImageNet are as follows:
\begin{itemize}
    \item \textbf{Undefended Models}: For ResNet-18/50, we use the pretrained models provided by \texttt{torchvision}. For Swin-B/L, we use the pretrained models provided in the official github repository\footnote{https://github.com/microsoft/Swin-Transformer}, with initial patch size of 4, window size of 7, and image size of 224. For ConvNext-B/L, we use the pretrained models provided in the official github repository\footnote{https://github.com/facebookresearch/ConvNeXt}.
    \item \textbf{Adversarially Trained Models}: For adversarially trained models, we use the model weights provided by Robustbench~\cite{croce2021robustbench}.
    \item \textbf{DiffPure Defended Models}: We apply the DiffPure~\cite{nie2022DiffPure} defense to the undefended models. We follow the implementations of the official github repository\footnote{https://github.com/NVlabs/DiffPure}. 
\end{itemize}
\subsection{Victim Models for Places365}
The implementation details for the victim models of Places365 are as follows:
\begin{itemize}
\item \textbf{Undefended Models}: We use the pretrained ResNet-18/50 and DenseNet-161 models provided by the official repository of Places365\footnote{https://github.com/CSAILVision/places365}.
    \item \textbf{DiffPure Defended Models}: We apply the DiffPure~\cite{nie2022DiffPure} defense to the undefended models. 
\end{itemize}
\section{More Quantitative Results}
\subsection{Effect of $\lambda$}
We show the effect of the Lagrangian multiplier $\lambda$ of Eq. (\textcolor{red}{6}) in~\Cref{tab:lambda}. A small $\lambda$ fails to regularize the output to satisfy the perceptual constraint, resulting in a high failure rate. We chose $\lambda=100$ since it achieves the lowest classification accuracy and failure rate.

\begin{table}[t]
    \centering
    %\setlength{\tabcolsep}{1.8mm}
    \scalebox{1.0}{\begin{tabular}{c|cccccc}
    \toprule
        $\lambda$ & 10 & 50 & 100 & 150 &  200 &  500 \\ \midrule
        Accuracy (\%)& 24.6 & 2.8 & \textbf{1.8} & \textbf{1.8} & \textbf{1.8}  & 2.2 \\
        Failure (\%) &  28.8 & 1.4 & \textbf{0.0} & 0.2 & 0.4  & 0.2 \\ 
        %LPIPS & 0.368 & 0.247 & 0.239 & 0.240 & 0.239 & 0.238 \\ 
        \bottomrule
    \end{tabular}}
    \caption{\textbf{Effect of $\lambda$.} We report the top-1 accuracy and the failure rate where the LPIPS bound is not satisfied.}
    \label{tab:lambda}
\end{table}

\subsection{Comparison with Neural Perceptual Attacks}
By applying the perceptual constraint, I2A becomes a special case of the neural perceptual attacks (NPA)~\cite{laidlaw2021perceptual}, which aims to find an adversarial example ${\vect{x}_\text{adv}}\in \gX$ with a perceptual bound $\gamma$ such that ${\vect{x}_\text{adv}}$ is perceptually similar to $\vect{x}$ but causes the classifier $f$ to misclassify:
\begin{equation}
    f({\vect{x}_\text{adv}})\neq y,\quad\text{and}\quad d({\vect{x}_\text{adv}}, \vect{x})\leq \gamma,
    \label{eq:NPA}
\end{equation} 
where $d$ is the LPIPS distance, and $y$ is the ground truth label.~\cite{laidlaw2021perceptual} proposed the Lagrangian Perceptual Attack (LPA) to solve for ${\vect{x}_\text{adv}}$ by using a Lagrangian relaxation of the following constrained optimization problem:

\begin{equation}
    \max_{{\vect{x}_\text{adv}}} \mathcal{L}_m({\vect{x}_\text{adv}}, y),\  \text{s.t.},  d({\vect{x}_\text{adv}}, \vect{x}) \leq \gamma, 
    \label{eq:lpa}
\end{equation} 
where $\mathcal{L}_m$ is the margin loss from~\cite{carlini2017towards}. 

The main differences between LPA and I2A are as follows: 1) LPA is a \textit{noise-based } attack that generates $\vect{x}_\text{adv}$ by adding optimized adversarial noise to $\vect{x}$, while I2A is a \textit{semantic} attack that generates semantically meaningful perturbation and constraints $\vect{x}_\text{adv}$ to be \textit{on-manifold}; 2) The adversarial noise generated by LPA lacks interpretability and naturalness, while I2A generates \textit{interpretable} and \textit{natural} adversarial images; 2) I2A is a \textit{language-guided} attack that allows the user to control the adversarial perturbations through language instructions, while LPA does not provide such controllability and the resulting adversarial noise is purely driven by optimization. 

\input{tables/white-box-lpa}

We provide quantitative comparisons between I2A and LPA under white-box attacks in~\Cref{tab:wb-lpa}. We set the perceptual bound to 0.3 for LPA and use the default settings of the official github repository\footnote{https://github.com/cassidylaidlaw/perceptual-advex}. LPA demonstrates strong attack ability on both undefended and adversarially trained models, resulting in nearly zero classification accuracy. However, since LPA is a noise-based attack, the adversarial noise can be easily removed by DiffPure, resulting in much lower attack performance than I2A when the DiffPure defense is applied. We also apply the EOT+BPDA techniques for adaptively attacking DiffPure and the results are summarized in~\Cref{tab:bpda-lpa}. I2A achieves significantly better performance than LPA under the DiffPure defense, especially under the adaptive attack setting. In addition, I2A achieves much better transferability than LPA under black-box attacks, as shown in~\cref{fig:blackbox-ipa}. For example, I2A achieves an average of 39.90\% classification accuracy for adversarially trained models, which is 14.91 points lower than LPA. 




\begin{table}
\centering
\setlength{\tabcolsep}{2.0mm}
\scalebox{0.9}{\begin{tabular}{c|c| c c c} 
\toprule
Model & Adaptive & Clean & LPA & \textbf{I2A} \\
\midrule
\multirow{2}{*}{ResNet-18} & \ding{55} & 70.0 & \second{67.5} & \textbf{43.5} \\
 & \ding{51} & 70.0 & \second{34.0} & \textbf{7.0 }\\
 \midrule
\multirow{2}{*}{ResNet-50} & \ding{55} & 75.0 & \second{74.5} & \textbf{52.5} \\
 & \ding{51} &  75.0 & \second{46.0} &  \textbf{9.0}\\
 \midrule
\multirow{2}{*}{Swin-B} & \ding{55} & 80.0 & \second{75.0} & \textbf{52.0} \\
 & \ding{51} & 80.0 & \second{62.5} &  \textbf{20.5}\\
\bottomrule
\end{tabular}}
\caption{\textbf{DiffPure defense under adaptive and non-adaptive attacks}~\cite{nie2022DiffPure}. We report top-1 (\%) on ImageNet. }
\label{tab:bpda-lpa}
\end{table}

\input{figs/black-box-lpa}



\subsection{Performance of Each Prompt}
We report the detailed performance of each prompt used by I2A in~\Cref{tab:wb-prompt}. We use four manually written prompts and one GPT-4 generated prompt. The five prompts achieve similar performance, which suggests the performance I2A is not sensitive to the input prompt. The prompt \texttt{"make it a vintage photo"} achieves slightly better performance compared to the others in terms of average accuracy.  
\input{tables/white-box-supp}



\section{More Visualization Results}
We provide more visualization results on ImageNet~\cite{deng2009imagenet} in~\cref{fig:vis_supp-2,fig:vis_supp}. We also provide visualization results on Places365~\cite{zhou2017places} in~\cref{fig:vis_places,fig:vis_places2}. I2A generates diverse and natural adversarial images based on the language instructions, and generalizes well to different datasets.

\input{figs/vis_supp_2}
\input{figs/vis_supp}
\input{figs/vis_places}
\input{figs/vis_places2}
\section{Prompt for GPT-4}
In this work, we propose to automatically generate image-specific editing instructions by first using BLIP-2~\cite{li2023blip} to generate image captions and feed them into GPT-4~\cite{openai2023gpt}. We utilize few-shot in-context learning by presenting 50 manually written examples in the prompt without fine-tuning the GPT-4 model. The prompt for GPT-4 to generate the edit instructions is presented in~\Cref{tab:gpt_prompt}.
\input{tables/prompt}



==> tables/white-box-v2.tex <==
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{0.9mm}
\scalebox{0.9}{\begin{tabular}{c | l | c c c c c c c c c c c | c} 
\hline
Model & Method & Clean & FGSM & PGD & MIM & Auto & Fog & Gabor & Elastic & Snow & StAdv & PerC-AL  & \textbf{I2A (Ours)} \\
\hline
\multirow{3}{*}{\rotatebox{0}{ResNet-18}} & Undefended &69.68        & 0.90  & {0.00}  & {0.00}  & 0.00      & 5.24  & 0.20  & {0.12}    & 0.26  & 0.00 & 56.16   & 1.20 \\
 & Salman2020~\cite{salman2020adversarially} & 52.92        & 32.54 & 29.77 & 29.84 & 25.32      & 27.14 & 33.44 & 30.40   & 30.46 & 29.40 & \second{9.92}    & \best{0.54} \\
  %& JPG~\cite{dziugaite2016study}  & 67.96        & 2.22  & \second{0.12}  & 0.00 & 1.88       & 20.96 & \second{0.12}  & 3.36    & 1.24  & 0.00 & 62.34   & 18.79\\
  %& Smoothing~\cite{xu2017feature}& 65.86        & 6.84  & 3.58  & \second{1.78}  & 7.80       & 22.06 & \best{1.62}  & 15.52   & 5.16  & 3.10  & 63.70   & 25.68\\
  & DiffPure~\cite{nie2022DiffPure} & 64.70        & 58.98 & 62.16 & 61.36 & 63.22 &  51.20 & 59.84 & 54.56 & 53.34 & \second{49.58} & 64.74 & \best{42.47}\\
 \hline
\multirow{5}{*}{\rotatebox{0}{ResNet-50}} & Undefended & 76.52        & 5.96  & 0.00 & 0.00 & 0.00      & 6.76  & {0.04}  & 0.52    & 1.12  & 0.00 & 72.34   & 2.11 \\
 & Salman2020~\cite{salman2020adversarially} & 64.02        & 43.44 & 38.98 & 39.06 & 34.96      & 36.22 & 41.44 & 40.36   & 40.36 & 36.56 & \second{18.68}   & \best{1.42}   \\
 & Engstrom2019~\cite{engstrom2019learning}  & 62.56        & 39.92 & 32.92 & 33.18 & 29.22      & 37.30 & 37.24 & 38.18   & 37.94 & 36.46 & \second{20.96}   & \best{2.52}  \\
 & FastAT~\cite{Wong2020Fast} & 55.62        & 32.84 & 27.94 & 26.26 & 26.24      & 19.54 & 30.76 & 31.32   & 27.28 & 31.90 & \second{13.74}   & \best{1.29}  \\
  % & JPG~\cite{dziugaite2016study} & 74.72        & 10.44 & 2.62  & 0.64  & 5.02       & 33.94 & \second{0.20}  & 9.26    & 4.92  & \best{0.08}  & 73.32   & 24.59 \\
  % & Smoothing~\cite{xu2017feature}& 71.80        & 17.68 & 12.40 & \second{5.78}  & 17.70      & 32.56 & \best{2.88}  & 25.84   & 11.26 & 7.10  & 71.44   & 30.48\\
    & DiffPure~\cite{nie2022DiffPure} & 70.54        & 66.94 & 69.16 & 68.06 & 69.68 &  58.90 & 66.42 & 62.98 & 61.62 & \second{56.20}  & 70.48 & \best{46.87}\\
 \hline
\multirow{4}{*}{\rotatebox{0}{ConvNeXt-B}} & Undefended & 83.36        & 41.44 & 0.00  & 0.00  & 0.00       & 11.16 & 0.14  & 7.26    & 6.86  & 0.70  & 19.94   & 8.93  \\
 & ARES~\cite{liu2023comprehensive} & 76.02        & 59.60 & 56.28 & 56.60 & 55.82      & 59.41 & 58.06 & 54.78   & 59.36 & \second{47.56} & 74.66   & \best{4.12}  \\
 & ConvStem~\cite{singh2023revisiting} & 75.90        & 59.92 & 56.74 & 56.88 & 56.14      & 60.12 & 58.64 & 55.32   & 59.32 & \second{49.56} & 75.22   & \best{3.62} \\
   % & JPG~\cite{dziugaite2016study}& 82.40        & 45.22 & 46.36 & 30.90 & 52.74      & 61.38 & \best{7.74}  & 36.38   & 37.24 & \second{12.78} & 38.44   & 39.33\\
 % & Smoothing~\cite{xu2017feature}& 80.10        & 49.10 & 50.74 & 38.94 & 55.76      & 40.58 & 16.72 & 46.74   & 35.64 & 39.52 & 60.02   & 42.86\\
    & DiffPure~\cite{nie2022DiffPure}& 78.10        & 74.90 & 77.32 & 76.58 & 77.54 &  69.28 & 75.04 & 70.70 & \second{54.82} & 70.92 & 75.74 & \best{53.34}  \\
    \hline
\multirow{4}{*}{\rotatebox{0}{ConvNeXt-L}} & Undefended & 83.62        & 44.44 & 0.00  & 0.00  & 0.00       & 9.38  & 0.18  & 8.62    & 6.72  & 1.60  & 16.08   & 9.32  \\
 & ARES~\cite{liu2023comprehensive} & 78.02        & 62.00 & 58.60 & 58.76 & 58.48      & 60.52 & 60.78 & 57.40   & 61.74 & \second{51.22} & 77.02   & \best{4.95}\\
 & ConvStem~\cite{singh2023revisiting} & 77.00        & 60.58 & 57.70 & 58.00 & 57.70      & 60.28 & 59.96 & 56.58   & 60.54 & \second{49.22} & 76.62   & \best{4.91}\\
   %  & JPG~\cite{dziugaite2016study}& 82.64        & 48.92 & 48.36 & 34.50 & 55.02      & 61.14 & \best{9.14}  & 38.74   & 38.78 & \second{16.06} & 38.34   & 39.17\\
 % & Smoothing~\cite{xu2017feature}& 81.40        & 52.12 & 50.44 & 39.86 & 55.52      & 34.60 & \best{15.92} & 49.84   & \second{33.32} & 44.66 & 60.48   & 41.73\\
    & DiffPure~\cite{nie2022DiffPure}& 78.68        & 75.12 & 77.84 & 77.02 &     78.12 &  \second{69.84}	& 75.32	& 71.44	& 73.66 & 71.52 & 78.12 & \best{52.71} \\
  \hline
\multirow{3}{*}{\rotatebox{0}{Swin-B}} & Undefended & 81.98        & 43.50 & 0.00  & 0.00  & 0.00       & 12.24 & 0.30  & 6.34    & 6.64  & 2.52  & 51.02   & 8.81  \\
 & ARES~\cite{liu2023comprehensive} & 76.16        & 59.78 & 57.12 & 57.32 & 56.16      & 59.18 & 58.76 & 54.94   & 58.90 & 47.76 & \second{41.06}   & \best{3.47}\\
   %  & JPG~\cite{dziugaite2016study}& 79.20        & 48.46 & 54.88 & 37.04 & 57.78      & 63.16 & \second{18.50} & 40.30   & 41.74 & \best{18.36} & 67.88   & 38.49\\
  % & Smoothing~\cite{xu2017feature}& 78.53        & 52.18 & 59.92 & 46.68 & 62.34      & 52.80 & \best{23.94} & 52.00   & 41.64 & 45.62 & 74.72   & \second{41.54}\\
    & DiffPure~\cite{nie2022DiffPure} & 76.60        & 74.02 & 75.88 & 75.28 &       75.92 & \second{68.64}	& 73.50	& 70.40	& 70.90  & 70.12 &  76.54 & \best{50.65}\\
  \hline
\multirow{3}{*}{\rotatebox{0}{Swin-L}} & Undefended & 85.06        & 45.72 & 0.00  & 0.00  & 0.00       & 6.92  & 0.78  & 4.46    & 8.72  & 2.96  & 57.62   & 8.40 \\
 & ARES~\cite{liu2023comprehensive} & 78.92        & 62.84 & 59.44 & 59.72 & 59.56      & 60.82 & 61.60 & 57.88   & 62.34 & \second{51.62} & 62.56   & \best{4.98}  \\
   %  & JPG~\cite{dziugaite2016study} & 82.82        & 55.42 & 63.04 & 45.02 & 67.2       & 71.68 & \best{25.18} & 54.62   & 51.8  & \second{28.12} & 73.38   & 44.11\\
 %  & Smoothing~\cite{xu2017feature}& 82.86        & 59.02 & 63.84 & 51.08 & 66.34      & 62.86 & 34.46 & 63.34   & 52.64 & 55.30 & 80.06   & \best{46.24}\\
    & DiffPure~\cite{nie2022DiffPure} & 81.40         & 79.56 & 80.66 & 80.26 &  81.02 &   \second{73.56}	& 78.72	& 75.5 & 75.9  & 74.48 &  80.92 & \best{55.18}\\
  \hline
\multicolumn{2}{c|}{Average Accuracy} & 73.97 & 51.13 & 41.75 & 41.55 & 41.14 & 41.98 & 42.33 & 41.37 & 41.76 & \second{37.81} & 54.00 & \best{16.90}\\ \hline
%\multicolumn{2}{c|}{Average FID $\downarrow$} \\ \hline
\end{tabular}}
\caption{Classification accuracy (\%) under white-box attacks on ImageNet. The best performance of each defense method is marked in \best{{dark blue}} and the second best is in \second{{light blue}}. }
\label{tab:wb}
\end{table*}


==> tables/white-box.tex <==
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{0.9mm}
\begin{tabular}{c | l | c c c c c c c c c c c | c} 
\hline
Model & Method & Clean & FGSM & PGD & MIM & Auto & Fog & Gabor & Elastic & Snow & StAdv & PerC-AL  & I2A (Ours) \\
\hline
\multirow{5}{*}{\rotatebox{90}{ResNet-18}} & Undefended &69.68        & 0.90  & 0.00  & 0.00  & 0.00       & 5.24  & 0.20  & 0.12    & 0.26  & 0.00  & 56.16   & 1.20 \\
 & Salman2020~\cite{salman2020adversarially} & 52.92        & 32.54 & 29.77 & 29.84 & 25.32      & 27.14 & 33.44 & 30.40   & 30.46 & 29.40 & \second{9.92}    & \best{0.54} \\
  & JPG~\cite{dziugaite2016study}  & 67.96        & 2.22  & \second{0.12}  & \best{0.00}  & 1.88       & 20.96 & \second{0.12}  & 3.36    & 1.24  & \best{0.00}  & 62.34   & 18.79\\
  & Smoothing~\cite{xu2017feature}& 65.86        & 6.84  & 3.58  & \second{1.78}  & 7.80       & 22.06 & \best{1.62}  & 15.52   & 5.16  & 3.10  & 63.70   & 25.68\\
  & DiffPure~\cite{nie2022DiffPure} & 64.70        & 58.98 & 62.16 & 61.36 &            &       &       &         &       & 49.58 &         & \best{42.47}\\
 \hline
\multirow{7}{*}{\rotatebox{90}{ResNet-50}} & Undefended & 76.52        & 5.96  & 0.00  & 0.00  & 0.00       & 6.76  & 0.04  & 0.52    & 1.12  & 0.00  & 72.34   & 2.11 \\
 & Salman2020~\cite{salman2020adversarially} & 64.02        & 43.44 & 38.98 & 39.06 & 34.96      & 36.22 & 41.44 & 40.36   & 40.36 & 36.56 & \second{18.68}   & \best{1.42}   \\
 & Engstrom2019~\cite{engstrom2019learning}  & 62.56        & 39.92 & 32.92 & 33.18 & 29.22      & 37.30 & 37.24 & 38.18   & 37.94 & 36.46 & \second{20.96}   & \best{2.52}  \\
 & FastAT~\cite{Wong2020Fast} & 55.62        & 32.84 & 27.94 & 26.26 & 26.24      & 19.54 & 30.76 & 31.32   & 27.28 & 31.90 & \second{13.74}   & \best{1.29}  \\
   & JPG~\cite{dziugaite2016study} & 74.72        & 10.44 & 2.62  & 0.64  & 5.02       & 33.94 & \second{0.20}  & 9.26    & 4.92  & \best{0.08}  & 73.32   & 24.59 \\
  & Smoothing~\cite{xu2017feature}& 71.80        & 17.68 & 12.40 & \second{5.78}  & 17.70      & 32.56 & \best{2.88}  & 25.84   & 11.26 & 7.10  & 71.44   & 30.48\\
    & DiffPure~\cite{nie2022DiffPure} & 70.54        & 66.94 & 69.16 & 68.06 &            &       &       &         &       & 56.2  &         & \best{46.87}\\
 \hline
\multirow{6}{*}{\rotatebox{90}{ConvNeXt-B}} & Undefended & 83.36        & 41.44 & 0.00  & 0.00  & 0.00       & 11.16 & 0.14  & 7.26    & 6.86  & 0.70  & 19.94   & 8.93  \\
 & ARES~\cite{liu2023comprehensive} & 76.02        & 59.60 & 56.28 & 56.60 & 55.82      & 59.41 & 58.06 & 54.78   & 59.36 & \second{47.56} & 74.66   & \best{4.12}  \\
 & CvSt~\cite{singh2023revisiting} & 75.90        & 59.92 & 56.74 & 56.88 & 56.14      & 60.12 & 58.64 & 55.32   & 59.32 & \second{49.56} & 75.22   & \best{3.62} \\
    & JPG~\cite{dziugaite2016study}& 82.40        & 45.22 & 46.36 & 30.90 & 52.74      & 61.38 & \best{7.74}  & 36.38   & 37.24 & \second{12.78} & 38.44   & 39.33\\
  & Smoothing~\cite{xu2017feature}& 80.10        & 49.10 & 50.74 & 38.94 & 55.76      & 40.58 & 16.72 & 46.74   & 35.64 & 39.52 & 60.02   & 42.86\\
    & DiffPure~\cite{nie2022DiffPure}& 78.10        & 74.90 & 77.32 & 76.58 &            &       &       &         &       & 70.92 &         & 53.34  \\
    \hline
\multirow{6}{*}{\rotatebox{90}{ConvNeXt-L}} & Undefended & 83.62        & 44.44 & 0.00  & 0.00  & 0.00       & 9.38  & 0.18  & 8.62    & 6.72  & 1.60  & 16.08   & 9.32  \\
 & ARES~\cite{liu2023comprehensive} & 78.02        & 62.00 & 58.60 & 58.76 & 58.48      & 60.52 & 60.78 & 57.40   & 61.74 & \second{51.22} & 77.02   & \best{4.95}\\
 & CvSt~\cite{singh2023revisiting} & 77.00        & 60.58 & 57.70 & 58.00 & 57.70      & 60.28 & 59.96 & 56.58   & 60.54 & \second{49.22} & 76.62   & \best{4.91}\\
     & JPG~\cite{dziugaite2016study}& 82.64        & 48.92 & 48.36 & 34.50 & 55.02      & 61.14 & \best{9.14}  & 38.74   & 38.78 & \second{16.06} & 38.34   & 39.17\\
  & Smoothing~\cite{xu2017feature}& 81.40        & 52.12 & 50.44 & 39.86 & 55.52      & 34.60 & \best{15.92} & 49.84   & \second{33.32} & 44.66 & 60.48   & 41.73\\
    & DiffPure~\cite{nie2022DiffPure}& 78.68        & 75.12 & 77.84 & 77.02 &            &       &       &         &       & 71.52 &         & 52.71 \\
  \hline
\multirow{5}{*}{\rotatebox{90}{Swin-B}} & Undefended & 81.98        & 43.50 & 0.00  & 0.00  & 0.00       & 12.24 & 0.30  & 6.34    & 6.64  & 2.52  & 51.02   & 8.81  \\
 & ARES~\cite{liu2023comprehensive} & 76.16        & 59.78 & 57.12 & 57.32 & 56.16      & 59.18 & 58.76 & 54.94   & 58.90 & 47.76 & \second{41.06}   & \best{3.47}\\
     & JPG~\cite{dziugaite2016study}& 79.20        & 48.46 & 54.88 & 37.04 & 57.78      & 63.16 & \second{18.50} & 40.30   & 41.74 & \best{18.36} & 67.88   & 38.49\\
  & Smoothing~\cite{xu2017feature}& 78.53        & 52.18 & 59.92 & 46.68 & 62.34      & 52.80 & \best{23.94} & 52.00   & 41.64 & 45.62 & 74.72   & \second{41.54}\\
    & DiffPure~\cite{nie2022DiffPure} & 76.60        & 74.02 & 75.88 & 75.28 &            &       &       &         &       & 70.12 &         & 50.65\\
  \hline
\multirow{5}{*}{\rotatebox{90}{Swin-L}} & Undefended & 85.06        & 45.72 & 0.00  & 0.00  & 0.00       & 6.92  & 0.78  & 4.46    & 8.72  & 2.96  & 57.62   & 8.40 \\
 & ARES~\cite{liu2023comprehensive} & 78.92        & 62.84 & 59.44 & 59.72 & 59.56      & 60.82 & 61.60 & 57.88   & 62.34 & \second{51.62} & 62.56   & \best{4.98}  \\
     & JPG~\cite{dziugaite2016study} & 82.82        & 55.42 & 63.04 & 45.02 & 67.2       & 71.68 & \best{25.18} & 54.62   & 51.8  & \second{28.12} & 73.38   & 44.11\\
  & Smoothing~\cite{xu2017feature}& 82.86        & 59.02 & 63.84 & 51.08 & 66.34      & 62.86 & 34.46 & 63.34   & 52.64 & 55.30 & 80.06   & \best{46.24}\\
    & DiffPure~\cite{nie2022DiffPure} & 81.4         & 79.56 & 80.66 & 80.26 &            &       &       &         &       & 74.48 &         & \best{55.18}\\
  \hline
\multicolumn{2}{c}{Average Accuracy $\downarrow$} \\ 
\multicolumn{2}{c}{Average FID $\downarrow$} \\ \hline
\end{tabular}
\caption{Classification accuracy (\%) and FID under white-box attacks on ImageNet.}
\label{tab:wb}
\end{table*}

